Holistic Adversarially Robust Pruning

Neural networks can be drastically shrunk in size by removing redundant parameters. While crucial for the deployment on resource-constraint hardware, oftentimes, compression comes with a severe drop in accuracy and lack of adversarial robustness. Despite recent advances, counteracting both aspects has only succeeded for moderate compression rates so far. We propose a novel method, HARP, that copes with aggressive pruning significantly better than prior work. For this, we consider the network holistically. We learn a global compression strategy that optimizes how many parameters (compression rate) and which parameters (scoring connections) to prune specific to each layer individually. Our method fine-tunes an existing model with dynamic regularization, that follows a step-wise incremental function balancing the different objectives. It starts by favoring robustness before shifting focus on reaching the target compression rate and only then handles the objectives equally. The learned compression strategies allow us to maintain the pre-trained model natural accuracy and its adversarial robustness for a reduction by 99% of the network original size. Moreover, we observe a crucial influence of non-uniform compression across layers.

==> figures/mad-test/resnet18-cifar10.tex <==
\begin{tikzpicture}
\begin{semilogxaxis}[
%log ticks with fixed point,
height=0.5\linewidth,
width=0.8\linewidth,
legend pos=outer north east,
enlarge x limits=0.02,
enlarge y limits=0.05,
grid=both,
grid style={dashed,gray!30},
smooth,
tension=0.0,
xlabel={Model Compression [$\times$]},
ylabel={Accuracy [\%]},
xmin=1,
xmax=1000,
ymin=30,
ymax=60,
xtick={1, 10, 100, 1000},
ytick={10, 30, 50, 70, 90},
xticklabels={$10^0$, $10^1$, $10^2$, $10^3$},
ytick={30, 40, 50, 60},
yticklabel style = {font=\fontsize{6}{6}\selectfont},
xticklabel style = {font=\fontsize{6}{6}\selectfont},
ylabel style = {font=\fontsize{7}{7}\selectfont, yshift=-4ex},
xlabel style = {font=\fontsize{7}{7}\selectfont, yshift=1ex},
%x tick label as interval
scale only axis,
legend image post style={scale=0.6},
legend style={at={(0.02, 0.05)}, font=\fontsize{9}{9}\selectfont, 
	anchor=south west, 
	legend columns=2, fill=white, draw=none, nodes={scale=0.6, transform 
		shape}, column sep=2pt, line width=0.8pt},
legend cell align={left}
]


%%%%%%%%%%%%% ResNet18 %%%%%%%%%%%%%

\addplot [mark=*, color=tertiarycolor, mark options={scale=0.6}, 
line width=0.6pt]
coordinates {
	(1, 53.3)
	(1.43, 54.7)
	(2, 54.8)
	(3.33, 54.6)
	(10, 52.6)
	(100, 45.1)
}; %\hydra

\addplot [mark=triangle*, color=primarycolor, mark options={scale=0.6, 
solid}, 
line width=0.8pt]
coordinates {
	(1, 53.3)
	(1.43, 50.2)
	(2, 50.3)
	(3.33, 51.3)
	(10, 50.9)
	(100, 40.3)
}; %\radmm

%\addplot [only marks, mark=diamond*, color=madcolor, mark 
%options={scale=0.6,	solid}, line 
%width=0.8pt]
%coordinates {
%	(1,	84.2)
%	(4, 82.7)
%}; %\mad

\addplot [mark=diamond*, color=madcolor, mark 
options={scale=0.6, 
solid}, line 
width=0.8pt]
coordinates {
	(1,	53.3)
	(1.43, 55.6)
	(2, 55.3)
	(3.33, 55.2)
	(10, 53.0)
	(100, 49.8)
}; %\mad

%\addplot [mark=square*, color=secondarycolor, mark options={scale=0.6}, 
%line width=0.6pt]
%coordinates {
%	(1, 84.2)
%	(1, 84.6)
%	(2, 84.5)
%	(3, 84.5)
%	(4, 85.2)
%	(5, 81.4)
%	(6, 77.4)
%}; %\ourmethod

\addplot [mark=square*, color=secondarycolor, mark 
options={scale=0.6}, 
line width=0.6pt]
coordinates {
	(1, 53.3)
	(1.43, 54.6)
	(2, 54.9)
	(3.33, 54.7)
	(10, 53.6)
	(100, 51.3)
	(500, 49.2)
	(1000, 40.9)
}; %\ourmethod

\end{semilogxaxis}

\end{tikzpicture}

==> res/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/bcsp-compare.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\newcommand{\mycsvreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\arch}{#1} \and \equal{\advtrain}{#2} \and 
	\equal{\rate}{#3},
%	late after line=\\
	]%
	{results/bcsp_compare.csv}%
	{}
	{
		& \bcspbfoa
		& \bcspbfaa
		& \harpbfoa
		& \harpbfaa
	}
}

\begin{bcsptable}{.9\linewidth}
	\midrule
	\multirow{3}{*}{\vgg}
	& \pgd
	\mycsvreader{vgg}{pgd}{0.1}
	\mycsvreader{vgg}{pgd}{0.01}
	\\
	& \trades
	\mycsvreader{vgg}{trades}{0.1}
	\mycsvreader{vgg}{trades}{0.01}
	\\
	& \mart
	\mycsvreader{vgg}{mart}{0.1}
	\mycsvreader{vgg}{mart}{0.01}
	\\
	\midrule
	\multirow{3}{*}{\resnet[18]}
	& \pgd
	\mycsvreader{resnet}{pgd}{0.1}
	\mycsvreader{resnet}{pgd}{0.01}
	\\
	& \trades
	\mycsvreader{resnet}{trades}{0.1}
	\mycsvreader{resnet}{trades}{0.01}
	\\
	& \mart
	\mycsvreader{resnet}{mart}{0.1}
	\mycsvreader{resnet}{mart}{0.01}
	\\
	\bottomrule
\end{bcsptable}

==> tables/cifar10_results.tex <==

\newcommand{\mycsvreader}[5]{%
	\csvreader[
	head to column names,
	filter = \equal{\arch}{#2} \and \equal{\at}{#3} \and 
	\equal{\rate}{#4} \and \equal{\acc}{#5}
	]%
	{#1}%
	{}
	{
		\hydrabf
		& \radmmbf
		& \harpbf
	}
}

\begin{resulttable}{\linewidth}
\midrule
%		\multirow{9}{*}{\rotatebox{90}{\cifar[10]}} & 
\multirow{9}{*}{\rotatebox{90}{\resnet[18]}} 
& \multirow{3}{*}{\pgd} 
& Clean
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{nat}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{nat}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{nat}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{nat} 
\\
&
& \fgsm
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{fgsm}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{fgsm}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{fgsm}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{fgsm}
\\
&
& \pgd-10
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{pgd}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{pgd} 
\\
&
& \cwinf
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{cw}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{cw}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{cw}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{cw} 
\\ \cmidrule{2-15}
%
& \multirow{3}{*}{\trades} 
& Clean
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{nat}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{nat}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{nat}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{nat}
\\
&
& \fgsm
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{fgsm}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{fgsm}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{fgsm}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{fgsm} 
\\
&
& \pgd-10
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{pgd}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{pgd} 
\\
&
& \cwinf
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{cw}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{cw}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{cw}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{cw} 
\\ \cmidrule{2-15}
%
& \multirow{3}{*}{\mart} 
& Clean
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{nat}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{nat}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{nat}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{nat} 
\\
&
& \fgsm
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{fgsm}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{fgsm}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{fgsm}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{fgsm}
\\
&
& \pgd-10
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{pgd}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{pgd} 
\\
&
& \cwinf
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{cw}
& \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{cw}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{cw}
& \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{cw} 
\\ \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{9}{*}{\rotatebox{90}{\vgg}} 
& \multirow{3}{*}{\pgd} 
& Clean
& \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.99}{nat}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.999}{nat}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.25}{nat}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.1}{nat} 
\\
&
& \pgd-10
& \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.99}{pgd}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.999}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.25}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.1}{pgd} 
\\
&
& \cwinf
& \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.99}{cw}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.999}{cw}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.25}{cw}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.1}{cw} 
\\ \cmidrule{2-15}
%
& \multirow{3}{*}{\trades} 
& Clean
& \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{nat}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{nat}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{nat}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{nat} 
\\
&
& \pgd-10
& \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{pgd}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{pgd} 
\\
&
& \cwinf
& \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{cw}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{cw}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{cw}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{cw} 
\\ \cmidrule{2-15}
%
& \multirow{3}{*}{\mart} 
& Clean
& \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{nat}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{nat}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{nat}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{nat} 
\\
&
& \pgd-10
& \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{pgd}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{pgd}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{pgd} 
\\
&
& \cwinf
& \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{cw}
& \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{cw}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{cw}
& \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{cw} 
\\ \bottomrule
\end{resulttable}

==> tables/cifar10_results_hydra.tex <==

\newcommand{\mycsvreader}[5]{%
	\csvreader[
    head to column names,
    head to column names prefix = COL,
	filter = \equal{\COLarch}{#2} \and \equal{\COLat}{#3} \and 
	\equal{\COLrate}{#4} \and \equal{\COLacc}{#5}
	]%
	{#1}%
	{}
	{
		& \COLhydrabf
		& \COLharpbfhydra
	}
}

\begin{hydraresulttable}{\linewidth}
\midrule
  \multirow{9}{*}{\rotatebox{90}{\resnet[18]}}
& \multirow{4}{*}{\makecell{\trades\\\num{81.30}\,/\,\num{53.21}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{nat} 
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{pgd} 
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{cw}
\\ \cmidrule{2-11}
& \multirow{4}{*}{\makecell{\mart\\\num{80.16}\,/\,\num{53.72}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{nat} 
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{pgd} 
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{cw} 
\\ \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
  \multirow{9}{*}{\rotatebox{90}{\vgg}} 
& \multirow{4}{*}{\makecell{\trades\\\num{80.18}\,/\,\num{49.72}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{nat}
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{pgd} 
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{cw}
\\ \cmidrule{2-11}
& \multirow{4}{*}{\makecell{\mart\\\num{73.44}\,/\,\num{51.51}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{nat}
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{pgd} 
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{cw} 
\\ \bottomrule
\end{hydraresulttable}

==> tables/cifar10_results_radmm.tex <==

\newcommand{\mycsvreader}[5]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLarch}{#2} \and \equal{\COLat}{#3} \and 
	\equal{\COLrate}{#4} \and \equal{\COLacc}{#5}
	]%
	{#1}%
	{}
	{
		& \COLradmmbf
		& \COLharpbfradmm
	}
}

\begin{radmmresulttable}{\linewidth}
\midrule
  \multirow{4}{*}{\rotatebox{90}{\resnet[18]}}
& \multirow{4}{*}{\makecell{\pgd\\\num{82.89}\,/\,\num{50.05}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{nat} 
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{pgd}
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{pgd}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{pgd}{0.1}{cw}
\\ \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%
  \multirow{4}{*}{\rotatebox{90}{\vgg}}
& \multirow{4}{*}{\makecell{\pgd\\\num{79.68}\,/\,\num{47.60}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.1}{nat}
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.1}{pgd}
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{pgd}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{pgd}{0.1}{cw}
\\ \bottomrule
\end{radmmresulttable}

==> tables/cifar10_results_radmm_res.tex <==

\newcommand{\mycsvreader}[5]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLarch}{#2} \and \equal{\COLat}{#3} \and 
	\equal{\COLrate}{#4} \and \equal{\COLacc}{#5}
	]%
	{#1}%
	{}
	{
		& \COLradmmbf
		& \COLharpbfradmm
	}
}

\begin{radmmresulttable}{\linewidth}
\midrule
  \multirow{8}{*}{\rotatebox{90}{\resnet[18]}}
& \multirow{4}{*}{\makecell{\trades\\\num{81.30}\,/\,\num{53.21}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{nat} 
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{pgd}
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{resnet}{trades}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{resnet}{trades}{0.1}{cw}
\\ \cmidrule{2-11}
& \multirow{4}{*}{\makecell{\mart\\\num{80.16}\,/\,\num{53.72}}}
& --
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{nat}
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{nat}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{nat}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{nat} 
\\
&
& \fgsm
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{fgsm}
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{fgsm}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{fgsm}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{fgsm}
\\
&
& \pgd-10
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{pgd}
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{pgd}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{pgd}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.99}{cw}
\mycsvreader{results/cifar10_weight.csv}{resnet}{mart}{0.999}{cw}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.25}{cw}
\mycsvreader{results/cifar10_channel.csv}{resnet}{mart}{0.1}{cw}
\\ \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%
  \multirow{8}{*}{\rotatebox{90}{\vgg}}
& \multirow{4}{*}{\makecell{\trades\\\num{80.18}\,/\,\num{49.72}}}
& --
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{nat}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{nat}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{nat}
\\
&
& \fgsm
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{fgsm}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{fgsm}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{fgsm}
\\
&
& \pgd-10
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{pgd}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{pgd}
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.99}{cw}
  \mycsvreader{results/cifar10_weight.csv}{vgg}{trades}{0.999}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.25}{cw}
  \mycsvreader{results/cifar10_channel.csv}{vgg}{trades}{0.1}{cw}
\\ \cmidrule{2-11}
& \multirow{4}{*}{\makecell{\mart\\\num{73.44}\,/\,\num{51.51}}}
& --
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{nat}
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{nat}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{nat}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{nat}
\\
&
& \fgsm
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{fgsm}
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{fgsm}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{fgsm}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{fgsm}
\\
&
& \pgd-10
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{pgd}
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{pgd}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{pgd}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.99}{cw}
\mycsvreader{results/cifar10_weight.csv}{vgg}{mart}{0.999}{cw}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.25}{cw}
\mycsvreader{results/cifar10_channel.csv}{vgg}{mart}{0.1}{cw}
\\
\bottomrule
\end{radmmresulttable}

==> tables/compare-channel-prune.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\setlength{\tabcolsep}{11pt}
\sisetup{
	input-open-uncertainty   = ,
	input-close-uncertainty  = ,
	input-signs              = + -,
}

\begin{tabular}{
	ccc
	S[table-format=1.2]
	%S[table-format=2.2]@{~/~}S[table-format=2.2]
	S[table-format=2.2]@{~}>{(~}S[table-format=2.2, table-space-text-pre={()},table-space-text-post={)}]<{)}
	%S[table-format=2.2]@{~/~}S[table-format=2.2]
	S[table-format=2.2]@{~}>{(~}S[table-format=2.2, table-space-text-pre={()},table-space-text-post={)}]<{)}
}
\toprule
  {\bf Method }
& {\bf Dataset }
& {\bf Model }
& {\bf x\flops }
& \multicolumn{2}{c}{\bf Accuracy }
& \multicolumn{2}{c}{\bf \pgd-Robustness }
\\
\midrule
% \multirow{3}{*}{DNR} & \multirow{2}{*}{\cifar[10]} & \vgg        & 2.00   & \bf 85.83 &     84.28   & 42.36 & \bf 44.82 \\
%                      &                             & \resnet[18] & 2.00   & \bf 87.49 &     87.37   & 48.33 & \bf 49.13 \\
% \cmidrule{2-8}
%                      & Tiny-\imagenet               & \vgg       & 1.45   & \bf 51.09 &     50.18   & 13.54 & \bf 15.49 \\
% \midrule
% \anpvs               & \cifar[10]                  & \vgg        & 2.41   &     88.18 & \bf 89.61   & 56.21 & \bf 57.02 \\
\multirow{3}{*}{DNR} & \multirow{2}{*}{\cifar[10]} & \vgg        & 2.00   &     85.83 &     +1.55   & 42.36 &     -2.46 \\
                     &                             & \resnet[18] & 2.00   &     87.49 &     +0.12   & 48.33 &     -0.80 \\
\cmidrule{2-8}
                     & Tiny-\imagenet               & \vgg       & 1.45   &     51.09 &     +0.91   & 13.54 &     -1.95 \\
\midrule
\anpvs               & \cifar[10]                  & \vgg        & 2.41   &     88.18 &     -1.43   & 56.21 &     -0.81 \\
\bottomrule
\end{tabular}


==> tables/imagenet_results_ch.tex <==
\newcommand{\mycsvreader}[3]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLattack}{#1} \and \equal{\COLpreg}{#2} \and 
	\equal{\COLprate}{#3}
	]%
	{results/imagenet_results.csv}%
	{}
	{
		& \COLradmmbf
		& \COLhydrabf
		& \COLharpbf
	}
}

\begin{imagenettable}{\linewidth}
	\midrule
	% \multirow{7}{*}{\rotatebox{90}{Channel Prune}} &
%	\multirow{4}{*}{\makecell{\bfseries Channel\\(\perc{50})}}
%	& -- 		\mycsvreader{nat}{channel}{0.5} \\
%	& \fgsm 	\mycsvreader{fgsm}{channel}{0.5} \\
%	& \pgd-10 	\mycsvreader{pgd}{channel}{0.5} \\
%	& \cwinf 	\mycsvreader{cw}{channel}{0.5}
%	\\ \midrule
	\multirow{4}{*}{\makecell{\bfseries Channel\\(\perc{90})}}
	& -- 		\mycsvreader{nat}{channel}{0.1} \\
	& \fgsm 	\mycsvreader{fgsm}{channel}{0.1} \\
	& \pgd-10 	\mycsvreader{pgd}{channel}{0.1} \\
	& \cwinf 	\mycsvreader{cw}{channel}{0.1} \\
	\bottomrule
	%	\multirow{7}{*}{\rotatebox{90}{Weight Prune}} 
	%	& \multirow{3}{*}{\perc{90}} 
	%	\mycsvreader{hydrabf}{weight}{0.1} \\
	%	& \mycsvreader{radmmbf}{weight}{0.1} \\ \cmidrule{3-7}
	%	& \mycsvreader{harpbf}{weight}{0.1}
	%	\\ \cmidrule{2-7}
	%	& \multirow{3}{*}{\perc{99}} 
	%	\mycsvreader{hydrabf}{weight}{0.01} \\ 
	%	& \mycsvreader{radmmbf}{weight}{0.01} \\ \cmidrule{3-7}
	%	& \mycsvreader{harpbf}{weight}{0.01}
	%	\\ \midrule
	
\end{imagenettable}

==> tables/imagenet_results_moderate.tex <==
\newcommand{\mycsvreader}[3]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLattack}{#1} \and \equal{\COLpreg}{#2} \and 
	\equal{\COLprate}{#3}
	]%
	{results/imagenet_results.csv}%
	{}
	{
		& \COLradmmbf
		& \COLhydrabf
		& \COLharpbf
	}
}

\begin{imagenetablemoderate}{\linewidth}
	\midrule
	% \multirow{7}{*}{\rotatebox{90}{Channel Prune}} & 
	\multirow{4}{*}{\makecell{\bfseries \freeat\\ 
	\num{60.25}\,/\,\num{32.82}}}
	& -- 		
	\mycsvreader{nat}{weight}{0.1} 
	& \mycsvreader{nat}{channel}{0.5}\\
	& \fgsm 	
	\mycsvreader{fgsm}{weight}{0.1} 
	& \mycsvreader{fgsm}{channel}{0.5}\\
	& \pgd-10 	
	\mycsvreader{pgd}{weight}{0.1} 
	& \mycsvreader{pgd}{channel}{0.5}\\
	& \cwinf
	\mycsvreader{cw}{weight}{0.1} 
	& \mycsvreader{cw}{channel}{0.5}\\
	\bottomrule
%	\multirow{7}{*}{\rotatebox{90}{Weight Prune}} 
%	& \multirow{3}{*}{\perc{90}} 
%	\mycsvreader{hydrabf}{weight}{0.1} \\
%	& \mycsvreader{radmmbf}{weight}{0.1} \\ \cmidrule{3-7}
%	& \mycsvreader{harpbf}{weight}{0.1}
%	\\ \cmidrule{2-7}
%	& \multirow{3}{*}{\perc{99}} 
%	\mycsvreader{hydrabf}{weight}{0.01} \\ 
%	& \mycsvreader{radmmbf}{weight}{0.01} \\ \cmidrule{3-7}
%	& \mycsvreader{harpbf}{weight}{0.01}
%	\\ \midrule

\end{imagenetablemoderate}

==> tables/imagenet_results_w.tex <==
\newcommand{\mycsvreader}[3]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLattack}{#1} \and \equal{\COLpreg}{#2} \and 
	\equal{\COLprate}{#3}
	]%
	{results/imagenet_results.csv}%
	{}
	{
		& \COLradmmbf
		& \COLhydrabf
		& \COLharpbf
	}
}

\begin{imagenettable}{\linewidth}
	\midrule
	% \multirow{7}{*}{\rotatebox{90}{Channel Prune}} & 
%	\multirow{4}{*}{\makecell{\bfseries Channel\\(\perc{90})}}
%	& -- 		\mycsvreader{nat}{weight}{0.1} \\
%	& \fgsm 	\mycsvreader{fgsm}{weight}{0.1} \\
%	& \pgd-10 	\mycsvreader{pgd}{weight}{0.1} \\
%	& \cwinf 	\mycsvreader{cw}{weight}{0.1}
%	\\ \midrule
	\multirow{4}{*}{\makecell{\bfseries Weight\\(\perc{99})}}
	& -- 		\mycsvreader{nat}{weight}{0.01} \\
	& \fgsm 	\mycsvreader{fgsm}{weight}{0.01} \\
	& \pgd-10 	\mycsvreader{pgd}{weight}{0.01} \\
	& \cwinf 	\mycsvreader{cw}{weight}{0.01} \\
	\bottomrule
%	\multirow{7}{*}{\rotatebox{90}{Weight Prune}} 
%	& \multirow{3}{*}{\perc{90}} 
%	\mycsvreader{hydrabf}{weight}{0.1} \\
%	& \mycsvreader{radmmbf}{weight}{0.1} \\ \cmidrule{3-7}
%	& \mycsvreader{harpbf}{weight}{0.1}
%	\\ \cmidrule{2-7}
%	& \multirow{3}{*}{\perc{99}} 
%	\mycsvreader{hydrabf}{weight}{0.01} \\ 
%	& \mycsvreader{radmmbf}{weight}{0.01} \\ \cmidrule{3-7}
%	& \mycsvreader{harpbf}{weight}{0.01}
%	\\ \midrule

\end{imagenettable}

==> tables/mad-compare-sparse90.tex <==
\begin{table}[tbh]
	\tablesize
	\setlength{\tabcolsep}{6pt}
	\begin{tabular}{clcccccccccc}
		\toprule
		\textbf{Model} & \textbf{Attack} & 
		\multicolumn{5}{c}{\textbf{\cifar[10]}} & 
		\multicolumn{5}{c}{\textbf{\svhn}} \\
		\cmidrule(lr){3-7}\cmidrule(lr){8-12}
		& 
		& \bf Adv. Train & \bf \radmms & \bf \hydra & \bf \mad & \bf 
		\ourmethod
		& \bf Adv. Train & \bf \radmms & \bf \hydra & \bf \mad & \bf 
		\ourmethod 
		\\
		\midrule
		\multirow{5}{*}{\vgg}
		& Clean
		& \num{81.33} & \num{79.02} & \num{76.38} & \num{81.43} & 
		\num{82.13}	
		& \num{93.17} & \num{92.41} & \num{87.93} & \num{92.80} & 
		\num{92.43}
		\\
		& \pgd-10
		& \num{50.24} & \num{47.43} & \num{47.36} & \num{51.81} & 
		\num{50.94}	
		& \num{56.04} & \num{54.88} & \num{54.62} & \num{58.43} & 
		\num{58.51}
		\\
		& \cwinf
		& \num{48.58} & \num{44.97} & \num{44.76} & \num{47.12} & 
		\num{47.35}	
		& \num{52.32} & \num{49.54} & \num{49.62} & \num{52.03} & \num{0}
		\\
		& \autopgd
		& \num{48.70} & \num{44.82} & \num{46.78} & \num{50.02} & 
		\num{48.25}	
		& \num{} & \num{} & \num{} & \num{} & \num{}
		%& \pgd-10
		%& \num{} & \num{} & \num{} & \num{} & \num{}	
		%& \num{} & \num{} & \num{} & \num{} & \num{}
		\\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/mad-compare.tex <==
\newcommand{\pretrainreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\method}{#1} \and \equal{\dataset}{#2} \and 
	\equal{\rate}{#3},
	%	late after line=\\
	]%
	{results/mad_compare.csv}%
	{}
	{
		& \txpre
	}
}

\newcommand{\prunereader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\method}{#1} \and \equal{\dataset}{#2} \and 
	\equal{\rate}{#3},
%	late after line=\\
	]%
	{results/mad_compare.csv}%
	{}
	{
		& \txpruned
		& \diff
	}
}

\begin{madcomparetable}{\linewidth}
		\midrule
%		\multirow{9}{*}{\rotatebox{90}{\cifar[10]}} &
		\multirow{2}{*}{\cifar[10]} &
		\mad
		\pretrainreader{mad}{cifar}{0.1} 
		\prunereader{mad}{cifar}{0.1}
		\prunereader{mad}{cifar}{0.01} \\
		&
		\ourmethod
		\pretrainreader{harp}{cifar}{0.1} 
		\prunereader{harp}{cifar}{0.1}
		\prunereader{harp}{cifar}{0.01} 
		\\ \midrule
		\multirow{2}{*}{\svhn} &
		\mad
		\pretrainreader{mad}{svhn}{0.1} 
		\prunereader{mad}{svhn}{0.1}
		\prunereader{mad}{svhn}{0.01} \\
		&
		\ourmethod
		\pretrainreader{harp}{svhn}{0.1} 
		\prunereader{harp}{svhn}{0.1}
		\prunereader{harp}{svhn}{0.01}
		\\
		\bottomrule
\end{madcomparetable}

==> tables/pretrain.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\setlength{\tabcolsep}{10pt}
\begin{tabular}{
		l
		wl{10mm}
		S[table-format=2.2]
		S[table-format=2.2]
		S[table-format=2.2]
		S[table-format=2.2]
		S[table-format=2.2]
		S[table-format=2.2]
	}
\toprule
  \multirow{2}{*}{\bf Model}
& \multirow{2}{*}{\bf Attack}
& \multicolumn{3}{c}{\bf \cifar[10] (Accuracy)}
& \multicolumn{3}{c}{\bf \svhn (Balanced Accuracy)}
\\ \cmidrule(lr){3-5} \cmidrule(lr){6-8}
& 
&{\bf \pgd} &{\centering \bf \trades} &{\centering \bf \mart}
&{\centering \bf \pgd} &{\centering \bf \trades} &{\centering \bf \mart}
\\ \midrule
\multirow{5}{*}{\resnet[18]}
& --
& 82.89 & 81.30 & 80.16		& 91.92 & 90.70 & 90.84 \\
& \pgd
& 50.05 & 53.21 & 53.72		& 56.82 & 57.12 & 59.53 \\
& \cwinf
& 47.95 & 50.60 & 48.53		& 52.41 & 51.40 & 51.48 \\
& \autopgd
& 47.78 & 51.88 & 51.59		& 47.67 & 45.60 & 51.25 \\
& \autoattack
& 45.30 & 49.48 & 46.39		& 43.56 & 42.08 & 42.93 \\
\midrule
\multirow{5}{*}{\vgg}
& --
& 79.68 & 80.18 & 73.44		& 91.38 & 88.66 & 87.45 \\
& \pgd
& 47.60 & 49.72 & 51.51		& 52.22 & 52.90 & 52.20 \\
& \cwinf
& 45.23 & 46.59 & 44.38		& 47.74 & 47.06 & 44.98 \\
& \autopgd
& 45.05 & 47.89 & 49.56		& 47.72 & 49.87 & 46.30 \\
& \autoattack
& 42.12 & 45.09 & 42.20		& 43.59 & 44.62 & 40.43 \\
\bottomrule
\end{tabular}


==> tables/rate-score-ch.tex <==

\newcommand{\mycsvreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\arch}{#2} \and \equal{\at}{#3},
	late after line=\\
	]%
	{#1}%
	{}
	{
		& \csuse{\at}
		& \oa
		& \aa
		& \rchoabf
		& \rchaabf
		& \schoabf
		& \schaabf
		& \hchoabf
		& \hchaabf
	}
}
\newcommand{\mymidrule}{\cmidrule(r){1-4}\cmidrule(l){5-10}}

\begin{influencetable3}{0.84\linewidth}
		\midrule
%		\multirow{9}{*}{\rotatebox{90}{\cifar[10]}} & 
		\multirow{3}{*}{\resnet[18]} 
		\mycsvreader{results/rate_score_cifar10.csv}{resnet}{pgd}  
		\mycsvreader{results/rate_score_cifar10.csv}{resnet}{trades}  
		\mycsvreader{results/rate_score_cifar10.csv}{resnet}{mart}
		\mymidrule
%		&
		\multirow{3}{*}{\vgg} 
		\mycsvreader{results/rate_score_cifar10.csv}{vgg}{pgd} 
		\mycsvreader{results/rate_score_cifar10.csv}{vgg}{trades} 
		\mycsvreader{results/rate_score_cifar10.csv}{vgg}{mart}
		\bottomrule
\end{influencetable3}

==> tables/rate-score-w.tex <==

\newcommand{\mycsvreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\arch}{#2} \and \equal{\at}{#3},
	late after line=\\
	]%
	{#1}%
	{}
	{
		& \csuse{\at}
		& \oa
		& \aa
		& \rwoabf
		& \rwaabf
		& \swoabf
		& \swaabf
		& \hwoabf
		& \hwaabf
	}
}
\newcommand{\mymidrule}{\cmidrule(r){1-4}\cmidrule(l){5-10}}

\begin{influencetable3}{0.84\linewidth}
		\midrule
%		\multirow{9}{*}{\rotatebox{90}{\cifar[10]}} & 
		\multirow{3}{*}{\resnet[18]} 
		\mycsvreader{results/rate_score_cifar10.csv}{resnet}{pgd}  
		\mycsvreader{results/rate_score_cifar10.csv}{resnet}{trades}  
		\mycsvreader{results/rate_score_cifar10.csv}{resnet}{mart}
		\mymidrule
%		&
		\multirow{3}{*}{\vgg} 
		\mycsvreader{results/rate_score_cifar10.csv}{vgg}{pgd} 
		\mycsvreader{results/rate_score_cifar10.csv}{vgg}{trades} 
		\mycsvreader{results/rate_score_cifar10.csv}{vgg}{mart}
		\bottomrule
\end{influencetable3}

==> tables/results_hydra.tex <==
\newcommand{\mycsvreader}[5]{%
	\csvreader[
    head to column names,
    head to column names prefix = COL,
	filter = \equal{\COLarch}{#2} \and \equal{\COLat}{#3} \and 
	\equal{\COLrate}{#4} \and \equal{\COLacc}{#5}
	]%
	{#1}%
	{}
	{
		& \COLhydrabf
		& \COLhydrastd
		& \COLharpbf
		& \COLharpstd
	}
}

\begin{hydrastdtableW}{\linewidth}
\midrule
  \multirow{15}{*}{\rotatebox{90}{\resnet[18]}}
& \multirow{5}{*}{\pgd}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\trades}
& --
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{nat}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{nat}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{nat}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{nat}
   
\\
&
& \pgd
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{pgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{pgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{pgd}
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{cw}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{cw}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{cw}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{cw}
   
\\
&
& \autopgd
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{autopgd}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{autopgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{autopgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\mart}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{autoattack}
\\ \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \multirow{15}{*}{\rotatebox{90}{\vgg}}
& \multirow{5}{*}{\pgd}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\trades}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\mart}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{autoattack}
\\ \bottomrule
\end{hydrastdtableW}

==> tables/results_radmm.tex <==
\newcommand{\mycsvreader}[5]{%
	\csvreader[
    head to column names,
    head to column names prefix = COL,
	filter = \equal{\COLarch}{#2} \and \equal{\COLat}{#3} \and 
	\equal{\COLrate}{#4} \and \equal{\COLacc}{#5}
	]%
	{#1}%
	{}
	{
		& \COLradmmHabf
		& \COLradmmstd
		& \COLharpRabf
		& \COLharpstd
	}
}

\begin{radmmstdtableW}{\linewidth}
\midrule
  \multirow{15}{*}{\rotatebox{90}{\resnet[18]}}
& \multirow{5}{*}{\pgd}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{pgd}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{pgd}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\trades}
& --
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{nat}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{nat}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{nat}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{nat}
   
\\
&
& \pgd
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{pgd}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{pgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{pgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{pgd}
\\
&
& \cwinf
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{cw}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{cw}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{cw}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{cw}
   
\\
&
& \autopgd
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{autopgd}
  \mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{autopgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{autopgd}
  \mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{trades}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{trades}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\mart}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{resnet}{mart}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{resnet}{mart}{0.999}{autoattack}
\\ \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \multirow{15}{*}{\rotatebox{90}{\vgg}}
& \multirow{5}{*}{\pgd}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{pgd}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{pgd}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\trades}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{trades}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{trades}{0.999}{autoattack}
\\ \cmidrule{2-19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multirow{5}{*}{\mart}
& --
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{nat}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{nat}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{nat}

\\
&
& \pgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{pgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{pgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{pgd}
\\
&
& \cwinf
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{cw}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{cw}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{cw}

\\
&
& \autopgd
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{autopgd}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{autopgd}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{autopgd}

\\
&
& \autoattack
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.99}{autoattack}
\mycsvreader{results/cifar10_weight_errorbar.csv}{vgg}{mart}{0.999}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.99}{autoattack}
\mycsvreader{results/svhn_weight_errorbar.csv}{vgg}{mart}{0.999}{autoattack}
\\ \bottomrule
\end{radmmstdtableW}

==> tables/stg-compare-hydra.tex <==
\newcommand{\myreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\method}{#1} \and \equal{\arch}{#2} \and 
	\equal{\prate}{#3},
	late after line=\\
	]%
	{results/lamp_erk_compare_cifar10.csv}%
	{}
	{	
		& \sparsity\perc{}
		& \erkoabf
		& \erkaabf
		& \lampoabf
		& \lampaabf
		& \harpoabf
		& \harpaabf
	}
}
\begin{subtable}{.49\linewidth}
	\caption{\vgg}
	\begin{stgcomparetable}{\linewidth}
		\midrule
		\myreader{hydra}{vgg}{0.01}
		\myreader{hydra}{vgg}{0.001}
		\bottomrule
	\end{stgcomparetable}
\end{subtable}
\hskip 5pt
\begin{subtable}{.49\linewidth}
	\caption{\resnet}
	\begin{stgcomparetable}{\linewidth}
		\midrule
		\myreader{hydra}{resnet}{0.01}
		\myreader{hydra}{resnet}{0.001}
		\bottomrule
	\end{stgcomparetable}
\end{subtable}

==> tables/stg-compare-radmm.tex <==
\newcommand{\myreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\method}{#1} \and \equal{\arch}{#2} \and 
	\equal{\prate}{#3},
	late after line=\\
	]%
	{results/lamp_erk_compare_cifar10.csv}%
	{}
	{	
		& \sparsity\perc{}
		& \erkoabf
		& \erkaabf
		& \lampoabf
		& \lampaabf
		& \harpoabf
		& \harpaabf
	}
}
\begin{subtable}{.49\linewidth}
	\caption{\vgg}
	\begin{stgcompareradmm}{\linewidth}
		\midrule
		\myreader{radmm}{vgg}{0.01}
		\myreader{radmm}{vgg}{0.001}
		\bottomrule
	\end{stgcompareradmm}
\end{subtable}
\hskip 5pt
\begin{subtable}{.49\linewidth}
	\caption{\resnet}
	\begin{stgcompareradmm}{\linewidth}
		\midrule
		\myreader{radmm}{resnet}{0.01}
		\myreader{radmm}{resnet}{0.001}
		\bottomrule
	\end{stgcompareradmm}
\end{subtable}

==> tables/stg-compare-resnet.tex <==
\newcommand{\myreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\method}{#1} \and \equal{\arch}{#2} \and 
	\equal{\prate}{#3},
	late after line=\\
	]%
	{results/lamp_erk_compare_cifar10.csv}%
	{}
	{	
		& \sparsity\perc{}
		& \erkoabf
		& \erkaabf
		& \lampoabf
		& \lampaabf
		& \harpoabf
		& \harpaabf
	}
}

\begin{stgcomparetable}{.5\linewidth}
	\midrule
	\myreader{hydra}{resnet}{0.01}
	\myreader{hydra}{resnet}{0.001}
	\bottomrule
\end{stgcomparetable}

==> tables/svhn_data_dist.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}


\tablesize
\begin{tabular}{
		l
		S[table-format=2.2]
		S[table-format=2.2]
		S[table-format=2.2]
		S[table-format=2.2]
		S[table-format=1.2]
		S[table-format=1.2]
		S[table-format=1.2]
		S[table-format=1.2]
		S[table-format=1.2]
		S[table-format=1.2]
	}
	\toprule
	\bf Dataset	& \multicolumn{10}{c}{\bf Amount of Samples per Class [\%]} \\ \cmidrule{2-11}
				&{\centering 1}&{\centering 2}&{\centering 3}
				&{\centering 4}&{\centering 5}&{\centering 6}
				&{\centering 7}&{\centering 8}&{\centering 9}
				&{\centering 10}\\
	\midrule
	Training	& 18.92	& 14.45	& 11.60	& 10.18	& 9.39	& 7.82	& 7.64	& 6.89	& 6.36	& 6.75	\\
	Test		& 19.59	& 15.94	& 11.07	& 9.69	& 9.16	& 7.59	& 7.76	& 6.38	& 6.13	& 6.70	\\	
	\bottomrule
\end{tabular}


==> tables/svhn_results_channel.tex <==
\newcommand{\mycsvreader}[4]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLarch}{#1} \and \equal{\COLat}{#2} \and 
	\equal{\COLrate}{#3} \and \equal{\COLacc}{#4}
	]%
	{results/svhn_channel.csv}%
	{}
	{
		& \COLradmmbf
		& \COLhydrabf
		& \COLharpbf
	}
}

\newcommand{\mymidrule}{\cmidrule{2-10}}

\begin{svhnchanneltable}{.96\linewidth}
	\midrule
	\multirow{12}{*}{\rotatebox{90}{\resnet[18]}}
	& \multirow{4}{*}{\makecell{\pgd\\\num{92.70}\,/\,\num{59.33}}}
	%& \multirow{4}{*}{\pgd}
	& --
	\mycsvreader{resnet}{pgd}{0.25}{nat} &
	\mycsvreader{resnet}{pgd}{0.1}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{pgd}{0.25}{fgsm} &
	\mycsvreader{resnet}{pgd}{0.1}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{pgd}{0.25}{pgd} &
	\mycsvreader{resnet}{pgd}{0.1}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{pgd}{0.25}{cw} &
	\mycsvreader{resnet}{pgd}{0.1}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\trades\\\num{92.48}\,/\,\num{65.70}}}
	%& \multirow{4}{*}{\trades}
	& --
	\mycsvreader{resnet}{trades}{0.25}{nat} &
	\mycsvreader{resnet}{trades}{0.1}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{trades}{0.25}{fgsm} &
	\mycsvreader{resnet}{trades}{0.1}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{trades}{0.25}{pgd} &
	\mycsvreader{resnet}{trades}{0.1}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{trades}{0.25}{cw} &
	\mycsvreader{resnet}{trades}{0.1}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\mart\\\num{92.01}\,/\,\num{62.46}}}
	%& \multirow{4}{*}{\mart}
	& --
	\mycsvreader{resnet}{mart}{0.25}{nat} &
	\mycsvreader{resnet}{mart}{0.1}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{mart}{0.25}{fgsm} &
	\mycsvreader{resnet}{mart}{0.1}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{mart}{0.25}{pgd} &
	\mycsvreader{resnet}{mart}{0.1}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{mart}{0.25}{cw} &
	\mycsvreader{resnet}{mart}{0.1}{cw} \\
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\midrule
	\multirow{12}{*}{\rotatebox{90}{\vgg}}
	& \multirow{4}{*}{\makecell{\pgd\\\num{92.40}\,/\,\num{55.09}}}
	%& \multirow{4}{*}{\pgd}
	& --
	\mycsvreader{vgg}{pgd}{0.25}{nat} &
	\mycsvreader{vgg}{pgd}{0.1}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{pgd}{0.25}{fgsm} &
	\mycsvreader{vgg}{pgd}{0.1}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{pgd}{0.25}{pgd} &
	\mycsvreader{vgg}{pgd}{0.1}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{pgd}{0.25}{cw} &
	\mycsvreader{vgg}{pgd}{0.1}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\trades\\\num{90.27}\,/\,\num{56.96}}}
	%& \multirow{4}{*}{\trades}
	& --
	\mycsvreader{vgg}{trades}{0.25}{nat} &
	\mycsvreader{vgg}{trades}{0.1}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{trades}{0.25}{fgsm} &
	\mycsvreader{vgg}{trades}{0.1}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{trades}{0.25}{pgd} &
	\mycsvreader{vgg}{trades}{0.1}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{trades}{0.25}{cw} &
	\mycsvreader{vgg}{trades}{0.1}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\mart\\\num{89.25}\,/\,\num{56.50}}}
	%& \multirow{4}{*}{\mart}
	& --
	\mycsvreader{vgg}{mart}{0.25}{nat} &
	\mycsvreader{vgg}{mart}{0.1}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{mart}{0.25}{fgsm} &
	\mycsvreader{vgg}{mart}{0.1}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{mart}{0.25}{pgd} &
	\mycsvreader{vgg}{mart}{0.1}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{mart}{0.25}{cw} &
	\mycsvreader{vgg}{mart}{0.1}{cw} \\
	\bottomrule
\end{svhnchanneltable}

==> tables/svhn_results_hydra.tex <==
%
%\newcommand{\mycsvreader}[5]{%
%	\csvreader[
%    head to column names,
%    head to column names prefix = COL,
%	filter = \equal{\COLarch}{#2} \and \equal{\COLat}{#3} \and 
%	\equal{\COLrate}{#4} \and \equal{\COLacc}{#5}
%	]%
%	{#1}%
%	{}
%	{
%		& \COLhydrabf
%		& \COLradmmbf
%		& \COLharpbf
%	}
%}
%
%\begin{svhnresulttable}{\linewidth}
%\midrule
%  \multirow{16}{*}{\rotatebox{90}{\resnet[18]}}
%% & \multirow{4}{*}{\makecell{\pgd\\\num{92.70}\,/\,\num{59.33}}}
%& \multirow{4}{*}{\makecell{Channel \\ (\perc{75})}}
%& --
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.25}{nat}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.25}{nat}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.25}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.25}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.25}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.25}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.25}{pgd}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.25}{pgd}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.25}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.25}{cw}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.25}{cw}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.25}{cw}
%\\ \cmidrule{2-12}
%& \multirow{4}{*}{\makecell{Channel \\ (\perc{90})}}
%& --
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.1}{nat}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.1}{nat}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.1}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.1}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.1}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.1}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.1}{pgd}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.1}{pgd}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.1}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_channel.csv}{resnet}{pgd}{0.1}{cw}
%\mycsvreader{results/svhn_channel.csv}{resnet}{trades}{0.1}{cw}
%\mycsvreader{results/svhn_channel.csv}{resnet}{mart}{0.1}{cw}
%\\ \cmidrule{2-12}
%& \multirow{4}{*}{\makecell{Weight \\ (\perc{99})}}
%& --
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.99}{nat}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.99}{nat}
%\mycsvreader{results/svhn_weight.csv}{resnet}{mart}{0.99}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.99}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.99}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{resnet}{mart}{0.99}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.99}{pgd}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.99}{pgd}
%\mycsvreader{results/svhn_weight.csv}{resnet}{mart}{0.99}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.99}{cw}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.99}{cw}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.99}{cw}
%\\ \cmidrule{2-12}
%& \multirow{4}{*}{\makecell{Weight \\ (\perc{99.9})}}
%& --
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.999}{nat}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.999}{nat}
%\mycsvreader{results/svhn_weight.csv}{resnet}{mart}{0.999}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.999}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.999}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{resnet}{mart}{0.999}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.999}{pgd}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.999}{pgd}
%\mycsvreader{results/svhn_weight.csv}{resnet}{mart}{0.999}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_weight.csv}{resnet}{pgd}{0.999}{cw}
%\mycsvreader{results/svhn_weight.csv}{resnet}{trades}{0.999}{cw}
%\mycsvreader{results/svhn_weight.csv}{resnet}{mart}{0.999}{cw}
%\\ \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\multirow{16}{*}{\rotatebox{90}{\vgg}}
%% & \multirow{4}{*}{\makecell{\pgd\\\num{92.70}\,/\,\num{59.33}}}
%& \multirow{4}{*}{\makecell{Channel \\ (\perc{75})}}
%& --
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.25}{nat}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.25}{nat}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.25}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.25}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.25}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.25}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.25}{pgd}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.25}{pgd}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.25}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.25}{cw}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.25}{cw}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.25}{cw}
%\\ \cmidrule{2-12}
%& \multirow{4}{*}{\makecell{Channel \\ (\perc{90})}}
%& --
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.1}{nat}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.1}{nat}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.1}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.1}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.1}{fgsm}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.1}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.1}{pgd}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.1}{pgd}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.1}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_channel.csv}{vgg}{pgd}{0.1}{cw}
%\mycsvreader{results/svhn_channel.csv}{vgg}{trades}{0.1}{cw}
%\mycsvreader{results/svhn_channel.csv}{vgg}{mart}{0.1}{cw}
%\\ \cmidrule{2-12}
%& \multirow{4}{*}{\makecell{Weight \\ (\perc{99})}}
%& --
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.99}{nat}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.99}{nat}
%\mycsvreader{results/svhn_weight.csv}{vgg}{mart}{0.99}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.99}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.99}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{vgg}{mart}{0.99}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.99}{pgd}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.99}{pgd}
%\mycsvreader{results/svhn_weight.csv}{vgg}{mart}{0.99}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.99}{cw}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.99}{cw}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.99}{cw}
%\\ \cmidrule{2-12}
%& \multirow{4}{*}{\makecell{Weight \\ (\perc{99.9})}}
%& --
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.999}{nat}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.999}{nat}
%\mycsvreader{results/svhn_weight.csv}{vgg}{mart}{0.999}{nat}
%\\
%&
%& \fgsm
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.999}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.999}{fgsm}
%\mycsvreader{results/svhn_weight.csv}{vgg}{mart}{0.999}{fgsm}
%
%\\
%&
%& \pgd-10
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.999}{pgd}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.999}{pgd}
%\mycsvreader{results/svhn_weight.csv}{vgg}{mart}{0.999}{pgd}
%\\
%&
%& \cwinf
%\mycsvreader{results/svhn_weight.csv}{vgg}{pgd}{0.999}{cw}
%\mycsvreader{results/svhn_weight.csv}{vgg}{trades}{0.999}{cw}
%\mycsvreader{results/svhn_weight.csv}{vgg}{mart}{0.999}{cw}
%\\
%\bottomrule
%\end{svhnresulttable}


\newcommand{\mycsvreader}[4]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLarch}{#1} \and \equal{\COLat}{#2} \and 
	\equal{\COLrate}{#3} \and \equal{\COLacc}{#4}
	]%
	{results/svhn_weight.csv}%
	{}
	{
		& \COLhydrabf
		& \COLradmmbf
		& \COLharpbf
	}
}

\begin{svhnweighttable}{.9\linewidth}
	\midrule
	\multirow{12}{*}{\rotatebox{90}{\resnet[18]}}
	% & \multirow{4}{*}{\makecell{\pgd\\\num{92.70}\,/\,\num{59.33}}}
	& \multirow{4}{*}{\pgd}
	& --
	\mycsvreader{resnet}{pgd}{0.99}{nat} 
	\mycsvreader{resnet}{pgd}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{pgd}{0.99}{fgsm}
	\mycsvreader{resnet}{pgd}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{pgd}{0.99}{pgd}
	\mycsvreader{resnet}{pgd}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{pgd}{0.99}{cw}
	\mycsvreader{resnet}{pgd}{0.999}{cw} \\
	\cmidrule{2-9}
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\trades}
	& --
	\mycsvreader{resnet}{trades}{0.99}{nat} 
	\mycsvreader{resnet}{trades}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{trades}{0.99}{fgsm}
	\mycsvreader{resnet}{trades}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{trades}{0.99}{pgd}
	\mycsvreader{resnet}{trades}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{trades}{0.99}{cw}
	\mycsvreader{resnet}{trades}{0.999}{cw} \\
	\cmidrule{2-9}
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\mart}
	& --
	\mycsvreader{resnet}{mart}{0.99}{nat} 
	\mycsvreader{resnet}{mart}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{mart}{0.99}{fgsm}
	\mycsvreader{resnet}{mart}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{mart}{0.99}{pgd}
	\mycsvreader{resnet}{mart}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{mart}{0.99}{cw}
	\mycsvreader{resnet}{mart}{0.999}{cw} \\
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\midrule
	\multirow{12}{*}{\rotatebox{90}{\vgg}}
	% & \multirow{4}{*}{\makecell{\pgd\\\num{92.70}\,/\,\num{59.33}}}
	& \multirow{4}{*}{\pgd}
	& --
	\mycsvreader{vgg}{pgd}{0.99}{nat} 
	\mycsvreader{vgg}{pgd}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{pgd}{0.99}{fgsm}
	\mycsvreader{vgg}{pgd}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{pgd}{0.99}{pgd}
	\mycsvreader{vgg}{pgd}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{pgd}{0.99}{cw}
	\mycsvreader{vgg}{pgd}{0.999}{cw} \\
	\cmidrule{2-9}
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\trades}
	& --
	\mycsvreader{vgg}{trades}{0.99}{nat} 
	\mycsvreader{vgg}{trades}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{trades}{0.99}{fgsm}
	\mycsvreader{vgg}{trades}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{trades}{0.99}{pgd}
	\mycsvreader{vgg}{trades}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{trades}{0.99}{cw}
	\mycsvreader{vgg}{trades}{0.999}{cw} \\
	\cmidrule{2-9}
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\mart}
	& --
	\mycsvreader{vgg}{mart}{0.99}{nat} 
	\mycsvreader{vgg}{mart}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{mart}{0.99}{fgsm}
	\mycsvreader{vgg}{mart}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{mart}{0.99}{pgd}
	\mycsvreader{vgg}{mart}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{mart}{0.99}{cw}
	\mycsvreader{vgg}{mart}{0.999}{cw} \\
	\bottomrule
\end{svhnweighttable}

==> tables/svhn_results_weight.tex <==
\newcommand{\mycsvreader}[4]{%
	\csvreader[
	head to column names,
	head to column names prefix = COL,
	filter = \equal{\COLarch}{#1} \and \equal{\COLat}{#2} \and 
	\equal{\COLrate}{#3} \and \equal{\COLacc}{#4}
	]%
	{results/svhn_weight.csv}%
	{}
	{
		& \COLradmmbf
		& \COLhydrabf
		& \COLharpbf
	}
}

\newcommand{\mymidrule}{\cmidrule{2-10}}

\begin{svhnweighttable}{0.96\linewidth}
	\midrule
	\multirow{12}{*}{\rotatebox{90}{\resnet[18]}}
	& \multirow{4}{*}{\makecell{\pgd\\\num{92.70}\,/\,\num{59.33}}}
	%& \multirow{4}{*}{\pgd}
	& --
	\mycsvreader{resnet}{pgd}{0.99}{nat} &
	\mycsvreader{resnet}{pgd}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{pgd}{0.99}{fgsm} &
	\mycsvreader{resnet}{pgd}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{pgd}{0.99}{pgd} &
	\mycsvreader{resnet}{pgd}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{pgd}{0.99}{cw} &
	\mycsvreader{resnet}{pgd}{0.999}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\trades\\\num{92.48}\,/\,\num{65.70}}}
	%& \multirow{4}{*}{\trades}
	& --
	\mycsvreader{resnet}{trades}{0.99}{nat} & 
	\mycsvreader{resnet}{trades}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{trades}{0.99}{fgsm} &
	\mycsvreader{resnet}{trades}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{trades}{0.99}{pgd} &
	\mycsvreader{resnet}{trades}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{trades}{0.99}{cw} &
	\mycsvreader{resnet}{trades}{0.999}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\mart\\\num{92.01}\,/\,\num{62.46}}}
	%& \multirow{4}{*}{\mart}
	& --
	\mycsvreader{resnet}{mart}{0.99}{nat} & 
	\mycsvreader{resnet}{mart}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{resnet}{mart}{0.99}{fgsm} &
	\mycsvreader{resnet}{mart}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{resnet}{mart}{0.99}{pgd} &
	\mycsvreader{resnet}{mart}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{resnet}{mart}{0.99}{cw} &
	\mycsvreader{resnet}{mart}{0.999}{cw} \\
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\midrule
	\multirow{12}{*}{\rotatebox{90}{\vgg}}
	& \multirow{4}{*}{\makecell{\pgd\\\num{92.40}\,/\,\num{55.09}}}
	%& \multirow{4}{*}{\pgd}
	& --
	\mycsvreader{vgg}{pgd}{0.99}{nat} &
	\mycsvreader{vgg}{pgd}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{pgd}{0.99}{fgsm} &
	\mycsvreader{vgg}{pgd}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{pgd}{0.99}{pgd} &
	\mycsvreader{vgg}{pgd}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{pgd}{0.99}{cw} &
	\mycsvreader{vgg}{pgd}{0.999}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\trades\\\num{90.27}\,/\,\num{56.96}}}
	%& \multirow{4}{*}{\trades}
	& --
	\mycsvreader{vgg}{trades}{0.99}{nat} &
	\mycsvreader{vgg}{trades}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{trades}{0.99}{fgsm} &
	\mycsvreader{vgg}{trades}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{trades}{0.99}{pgd} &
	\mycsvreader{vgg}{trades}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{trades}{0.99}{cw} &
	\mycsvreader{vgg}{trades}{0.999}{cw} \\
	\mymidrule
	%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{\makecell{\mart\\\num{89.25}\,/\,\num{56.50}}}
	%& \multirow{4}{*}{\mart}
	& --
	\mycsvreader{vgg}{mart}{0.99}{nat} &
	\mycsvreader{vgg}{mart}{0.999}{nat} \\
	& & \fgsm
	\mycsvreader{vgg}{mart}{0.99}{fgsm} &
	\mycsvreader{vgg}{mart}{0.999}{fgsm} \\
	& & \pgd
	\mycsvreader{vgg}{mart}{0.99}{pgd} &
	\mycsvreader{vgg}{mart}{0.999}{pgd} \\
	& & \cwinf
	\mycsvreader{vgg}{mart}{0.99}{cw} &
	\mycsvreader{vgg}{mart}{0.999}{cw} \\
	%\bottomrule
\end{svhnweighttable}
